Recursive Variable-Length State Compression for Multi-Core Software Model Checking

High-performance multi-core software typically uses concurrent data structures. Tests for such data structures have significantly smaller state spaces than the entire software, making it feasible to model check them. However, dynamic memory allocations on the heap complicate the use of standard fixed-length state vectors. In this paper, we introduce dtree, a concurrent compression tree data structure that compactly stores variable-length states while allowing partial state reconstruction and incremental updates without concretising states. It supports describing a state as a tree, allowing direct modeling of the heap. We implemented dtree in DMC, our multi-core model checker. We show that its performance approaches that of state-of-the-art model checkers for fixed-length states. For models with variable-length states, dtree is up to 2.9 times faster.

==> chapters/dtreesparse.tex <==
\subsection{Sparse Delta updates}

To expand upon delta updates, we introduce \emph{sparse delta updates}. When a vector is changed in multiple non-consecutive locations, a single, normal delta update is costly, as the unchanged parts would need to be reconstructed and reinserted as well. Applying multiple, normal delta updates would result in the desired vector to be inserted into the tree, but also any intermediate vector. Moreover, parts of the tree might be accessed multiple times instead of once.

Sparse delta updates remedy this by recursing the node tree only once, like a normal delta update, but applying multiple smaller updates as needed to the tree. The requirement we impose on the given sparse delta updates is that they are sorted by offset in ascending order. This allows efficient tracking which delta applies to the left sub-tree and which to the right.

%In the next section we will see the details regarding \code{deltaSparse()} when used recursively.

%Sparse delta updates remedies this by recursing the tree until there is only a single delta update that applies to the sub-tree. The requirement we impose on the given sparse delta updates is that they are sorted by offset in ascending order. This allows efficient tracking which delta applies to the left sub-tree and which to the right.

%\todo{algorithm}

%\todo{illustration}

\subsection{Recursive Sparse Delta updates}
% Other names: Multi-phase delta updates, 

\begin{mylisting}[!b]
\caption{Processes}%
\label{lst:dtree:multidelta}%
\centering%
%\begin{minipage}{14cm}
{\lstset{language=pseudo,style=pseudospecific}
\begin{lstlisting}
getNextStates(StateID rootID) {
IL^for(p in {0,1,...,sv.n}) {
IL|IL^hword o1 = @SV::p[p] // hword-offset to p[p] within the struct SV
IL|IL|hword o2 = @Process::i // hword-offset to i within the struct Process
IL|IL|word proc_i = MC.getRecursive(rootID, {o1, o2}, |proc_i|);
IL|IL|proc_i = (proc_i + 1) % 10;
IL>IL>MC.recursiveDeltaSparse(rootID, {o1, o2, i});
\end{lstlisting}}
%\end{minipage}
\end{mylisting}
%Recursive delta updates support \needs{growing states} that grow at offsets within the vector and not only at the end.
\emph{Recursive sparse delta} updates allow modifications of the state tree in one single operation. Even though delta updates already traverse the tree recursively, recursive delta updates perform an additional recursion. The extra recursion is due to that the data of the vector constructed by the first tree is used as an index to a second tree. This can be applied many times. The extra data needed per recursive delta update is the offsets within the vectors that form the indices to the next tree.

%This is an elegant combination of \collapse and the compression tree:

This can be seen as LTSmin's projection method to project certain parts of a state onto a smaller vector, but then for a selection of variables in a tree of states. \todo{is this clear? do I remove it or expand on it?}

%\begin{wrapfigure}{r}{.5\columnwidth}
%\centering%
%%\begin{minipage}{14cm}
%%\includegraphics{images/hashtable/openaddr_linear}
%\def\svgwidth{.75\columnwidth}
%\scalebox{.666666666}{\input{images/processes_mem.pdf_tex}}
%%\end{minipage}
%\caption{Every \vectorbox{coltwolight}{\phantom{X}} is a \code{StateID}}%
%\label{fig:dtree:processesmem}%
%\end{wrapfigure}

We will illustrate this by changing the example in \cref{lst:dtree:processes} to use recursive sparse delta updates instead. To do this, we need \code{doSomeStep} to actually do something, like performing \code{i = (i + 1) \% 10}. The resulting code can be found in \cref{lst:dtree:multidelta}. In lines 3 and 4 we obtain the offsets we need to traverse the state tree. In line 5 we obtain the current value of \code{i} of the \code{p}th process. In line 6 we perform the operation and in line 6 we submit the changed value. Lines 5, 6 and 7 correspond to lines 12, 13 and 16 of \cref{lst:dtree:processes}, respectively.

This saves obtaining the root state \emph{entirely}. When this is useful depends on the model, but this method allows for flexibility.
%Before we dive into the detail, we first show why this is useful.
Recursive delta updates map quite well to a state vector with an arbitrary number of processes, each with a resizing heap, stack and registers. This example uses only two levels instead of the supported arbitrary number, but it clearly illustrates the applicability.

%\todo{algorithm}

%\todo{compare to \collapse: SPIN's root state is also variable length}

%\subsubsection{Dynamic memory is easy}

%We can use the recursive sparse delta updates to easily allocate dynamic memory that can be accessed throughout the model in an easy fashion. The dynamic memory is simply a vector and pointers are offsets within that memory vector. This makes allocation simple as well: this simply extends the vector with the required size and returns the offset to it. Pointer arithmetic stays the same.

%\newpage

%\subsection{Bringing it all together}

%\todo{NOTE: I will remove this subsection and all further subsections in this section and move onto the experiments at this point. Saves a page.}

%\subsection{Key differences}
%\label{sec:laarmandiff}

%Because the approaches share a lot of techniques at the core, it is important to highlight the difference and why dtree can support arbitrary length vectors, whereas Laarman cannot.

%\subsubsection{Power of two split}
%\label{sec:laarmandiff:powertwo}

%If we would split left and right in the middle, like Laarman, we would store the same data multiple times, but cut up in different ways. This does not happen only at the leaves of the tree, but throughout the entire tree. For \cref{fig:dtree:abcd_map}, it would add the 4 mappings
%\vectorbox{coltwolight}{4}$\rightarrow$\vectorbox{coltwolight}{1c},
%\vectorbox{coltwolight}{5}$\rightarrow$\vectorbox{coltwolight}{de},
%\vectorbox{coltwolight}{6}$\rightarrow$\vectorbox{coltwolight}{5f},
%\vectorbox{coltwolight}{7}$\rightarrow$\vectorbox{coltwolight}{46}, instead of the 2 we added. This continues in \cref{fig:dtree:abcdefgh}. We add three mappings, which is the minimum for a partly new vector. Using split in the middle adds:
%\vectorbox{colone}{8}$\rightarrow$\vectorbox{colone}{ef},
%\vectorbox{colone}{9}$\rightarrow$\vectorbox{colone}{gh},
%\vectorbox{colone}{10}$\rightarrow$\vectorbox{colone}{89},
%\vectorbox{colone}{11}$\rightarrow$\vectorbox{colone}{3,10}. Here there are four needed because the mapping \vectorbox{colone}{8}$\rightarrow$\vectorbox{colone}{ef} was not in the tree yet, since the split in the middle caused \vectorbox{coltwolight}{de} and \vectorbox{coltwolight}{f} to be leaves, instead of \vectorbox{coltwolight}{cd} and \vectorbox{coltwolight}{ef} when \vectorbox{coltwolight}{abcdef} was inserted.
%
%Note that the two approaches are identical for vectors of a fixed length that is a power of 2. The only difference is the size of the buckets of the root map, where length and type information are stored in the dtree.

%\subsubsection{Assumption of the availability of complete states}
%\label{sec:laarmandiff:completestates}

%- StateID only has the advantage that it is more efficient in terms of the queues of states to be visited. In memory as well as performance. Memorywise, use the 41GB (17\%) increase in memory footprint. Performancewise, better work stealing algorithms can be made if the work item is only a word. \todo{explain more, possibly link to Tom's work on workstealing}

%\subsubsection{Size of the root map}
%\label{sec:laarmandiff:rootmap}


%\begin{figure}
%\centering%
%%\begin{minipage}{14cm}
%%\includegraphics{images/hashtable/openaddr_linear}
%\def\svgwidth{.899\columnwidth}
%\scalebox{1}{\input{images/abcdefgh.pdf_tex}}
%%\end{minipage}
%\caption{The vector \emph{abcdefgh} is added to \cref{fig:dtree:abcdef}. \todo{make nicer}}%
%\label{fig:dtree:abcdefgh}%
%\end{figure}



==> chapters/relatedwork.tex <==
\section{Related work}

\subsection{Related state space exploration tools}

\setlength{\floatsep}{10pt}%
\setlength{\textfloatsep}{10pt}%
\setlength{\intextsep}{10pt}%

\begin{table}[!t]
\rowcolors{2}{black!5!white}{black!10!white}%
\setlength{\extrarowheight}{2pt}%
\renewcommand{\arraystretch}{1.0}
\caption{Requirement comparison of storage components.}%
\label{tab:relatedwork:backends}%
\centering%
\scalebox{1}{\begin{tabular}{l@{}lcccc}%
\rowcolor{darkgray}
& \headcell{Storage}
& \headcell{R1}
& \headcell{R2}
& \headcell{R3}
& \headcell{R4}
\\

%& stdmap[CITE]
%& \checkmark
%& (\checkmark)
%& \checkmark
%&
%& \code{std::unordered\_map} with a mutex
%\\

& cchm~\cite{c71e99bcd01f48b99fdff1c495588533}
& \checkmark
& \checkmark
& \checkmark
&
\\

& \treedbs~\cite{DBLP:conf/spin/LaarmanP011}
&
& \checkmark
&
& \checkmark
\\

& \compacttree~\cite{DBLP:journals/isse/Laarman19}
&
& \checkmark
&
& \checkmark
\\

& \dtree
& \checkmark
& \checkmark
& \checkmark
& \checkmark
\\

\end{tabular}}%
\end{table}

\subsection{Related state storage components}

\Cref{tab:relatedwork:backends} lists a number of state storage components. One way to store variable-length states is using a concurrent hash map\cite{c71e99bcd01f48b99fdff1c495588533}, where each state is stored uncompressed. We will refer to this implementation as cchm: concurrent chaining hash map.

\subsection{treedbs: concurrent compression tree by Laarman}
\label{sec:background:laarman}

